Adversarial Learning for Neural Dialogue Generation

In this paper, drawing intuition from the Turing test, we propose using adversarial training for open-domain dialogue generation: the system is trained to produce sequences that are indistinguishable from human-generated dialogue utterances. We cast the task as a reinforcement learning (RL) problem where we jointly train two systems, a generative model to produce response sequences, and a discriminator---analagous to the human evaluator in the Turing test--- to distinguish between the human-generated dialogues and the machine-generated ones. The outputs from the discriminator are then used as rewards for the generative model, pushing the system to generate dialogues that mostly resemble human dialogues. In addition to adversarial training we describe a model for adversarial {\em evaluation} that uses success in fooling an adversary as a dialogue evaluation metric, while avoiding a number of potential pitfalls. Experimental results on several metrics, including adversarial evaluation, demonstrate that the adversarially-trained system generates higher-quality responses than previous baselines.

==> 03-RL1.tex <==
In this section, we describe in detail the components of the proposed adversarial reinforcement learning model. 
\subsection{Notations}
The learning system consists of two agents. 
We use $p$ to denote sentences generated from the first agent and  $q$ to denote sentences from the second. The two agents take turns talking with each other. A dialogue can be represented as an alternating sequence of sentences generated by the two agents: $U=\{p_1, q_1, p_2, q_2, ..., p_{i}, q_{i}\}$.  We view the generated sentences as actions that are taken according to a policy defined by an
encoder-decoder recurrent neural networks.
\subsection{The generative Model}
The generative model $G$ defines the
 policy that generates an utterance, namely $p_{i}=\{w_1,w_2,...,w_N\}$, 
  given the dialogue history, denoted $\pi(p_{i}|p_{i-1},q_{i-1})$\footnote{ We found that using more than 2 context yields very tiny performance boost.
We therefore approximate the dialogue history using the concatenation of two preceding utterances. }. 
The policy takes a similar form to \sts models in which the source input is first mapped to a vector representation using a recurrent net
and defines the probability of generating each token in the target using a softmax function:
\begin{equation}
\begin{aligned}
&\pi(p_{i}|p_{i-1},q_{i-1})=\\
&~~~~~~~~~\prod_{w_t\in p_{i}} \pi(w_t|w_1,...,w_{t-1},p_{i-1},q_{i-1})
\end{aligned}
\label{eq2}
\end{equation}
\subsection{The Discriminative Model}
The discriminative model $D$ is a binary classifier that takes as input a sequence of dialogue utterances
$U=\{p_1,q_1,...,p_i,q_i\}$
 and outputs a label indicating whether the input is generated by humans or machines.  

The input dialogue is encoded into a vector representation 
using a hierarchical encoder  \cite{li2015hierarchical,serban2016building}. 
To be specific, each utterance $p$ or $q$ is mapped to a vector representation $h_p$ or $h_q$ using LSTM \cite{hochreiter1997long}.
Another LSTM is put on sentence level, mapping the entire dialogue sequence to a single representation. This representation is fed to a 2-class softmax function, returning the probability of the input dialogue episode being a machine-generated dialogue
(denoted $D_0(U)$)
 or a human-generated dialogue  (denoted $D_1(U)$). 
\subsection{Policy Gradient Training}
 The key idea of the system is to push the generator to produce utterances that are indistinguishable from human dialogues. We use policy gradient to achieve such a goal, in which the 
score of current utterances being human-generated ones assigned by the discriminator
(i.e.,  $D_1(U)$)
 is used as rewards for the generated utterance(s), and the system is trained to maximize the expected reward of generated utterance(s):
 \begin{equation}
 J(\theta)=\mathbb{E}_{\pi}(D_1(U)|\theta)
 \label{lb1}
 \end{equation}
We use the REINFORCE algorithm \cite{williams1992simple}, which is one type of policy gradient method to optimize the system:
Given the input dialogue history $L$, the first bot generates a dialogue utterance $p_{i+1}$ by sampling from the policy. 
If we are doing single-term simulation, 
the concatenation of the generated utterance $p_{i+1}$ and input is fed to the discriminator. If we are doing multi-turn simulation, the second bot updates the dialogue history by adding $p_{i+1}$, and samples another sequence using from the policy given the updated dialogue history. 
The two bots take turns to 
take to each other (i.e.,
do the encoding-decoding) until the maximum number of simulation turn is reached. 
Then the discriminator assigns a score to the entire simulated dialogue. 
 The derivation of Eq. \ref{lb1} is approximated using likelihood ratios \cite{williams1992simple,glynn1990likelihood,aleksand1968stochastic}:
 \begin{equation}
\begin{aligned}
\nabla J(\theta)=\nabla\log \pi(U) [D_1(U)-b(L)]
\end{aligned}
\end{equation}
where $\pi(U)$ denotes the probability of generating the entire dialogue computed using Eq.\ref{eq2}. 
 $b(L)$ denotes the baseline value to reduce the variance of the estimate while keeping it unbiased. 
The baseline value is computed using a strategy similar to actor-critic algorithm  \cite{sutton1998reinforcement,degris2012model}, in which we train another neural network model (the critic) to estimate the value (or future reward) of current state (i.e., the dialogue history $L$) under current policy $\pi$. The critic network takes as input the dialogue history, transforms it to a vector representation using a hierarchical network and maps the representation to a scalar. The network is optimized based on the mean squared loss between the estimated reward and real reward $D_1(U)$.


The discriminator is simultaneously updated with the positive examples being the human generated dialogue that contains dialogue history $L$ and the negative examples being 
the machine-generated dialogues. 
\subsection{Training Details}
 For the first stage of training, we  pre-train the generative model by predicting target sequences given the dialogue history. We trained a  \sts model \cite{sutskever2014sequence}   
 with attention \cite{bahdanau2014neural,luong2015effective}\footnote{a two-layer \sts model with 512 units for each hidden layer. We followed protocols defined in \cite{sutskever2014sequence} such as gradient clipping, mini-batch and learning rate decay.} using the OpenSubtitles dataset.

We also pre-train the discriminator. To generate negative examples, 
we  decode   part of the training data. 
Half of the negative examples are generated using beam-search with mutual information reranking 
as described in \newcite{li2015diversity},
and the other half is generated from sampling. 

The generator and the discriminator are initialized using the pre-trained ones. 
A curriculum learning strategy  \cite{bengio2009curriculum}  is adopted
in which we gradually increase the number of simulated turns. 
We generate 3 turns at most.  


We find it  important to add the entropy of the policy  \cite{williams1991function,mnih2016asynchronous}. 
The gradient
of the full objective function includes the entropy
regularization term: 
\begin{equation}
\begin{aligned}
&\nabla J(\theta)=\nabla\log \pi(U) [D_1(U)-b(H)]+\nabla\beta H(U)\\
\end{aligned}
\end{equation}
We also use  label smoothing \cite{warde2016adversarial}
to smooth the reward from the discriminator. Namely, instead of using $D_1(U)$ which is the probability of current input being a human-generated one, we use smoothed reward $D(U)$ given as follows:
$$D(U)=\alpha D_1(U)+(1-\alpha)D_0(U)$$
where $\alpha$ is set to $0.9$ as suggested by \newcite{salimans2016improved}. 
We also add an historical averaging part \cite{brown1951iterative,salimans2016improved} as a regularizer to smooth training:
 \begin{equation}
L= ||\theta-\frac{1}{t}\sum_{t}\theta_t ||^2
 \end{equation}
where $\theta_t$ denotes the value of the parameters at past time $t$. The historical average of the parameters is updated after each parameter update. 
  
For 
data-processing, 
model training and decoding  (both the proposed adversarial training model and the standard \sts models), we list a few  strategies (tricks) that  improve response quality, including: (1) Set a threshold and  remove all training examples with responses shorter than the threshold (the threshold is set to 4 in this paper). (2) Instead of using the same learning rate for all examples, using a weighted learning rate that considers the average tf-idf score for tokens within the response.
Such a strategy
 decreases the influence from the dull and generic utterances.\footnote{We treat each sentence as a document. Stop words are removed.} (3) Penalizing intra-sibling ranking when doing beam search decoding to promote N-best list diversity.  (4) Penalizing the language model score for the first decoded word as described in \newcite{li2015diversity}. (5) Penalizing word types that have already been generated. Such a strategy dramatically decreases the rate of repetitive responses such as {\it no. no. no. no. no.} or controversial responses such as {\it I don't like oranges but i like oranges}. 

\section{Adversarial Evaluation}
 The idea of adversarial evaluation is first proposed in 
\newcite{bowman2015generating} to 
train a discriminant
function
 to separate  generated and
true sentences, in an attempt to evaluate the model's sentence generation capability.
This  idea  also resembles  the Turing test 
which requires a human evaluator 
to distinguish  machine generated texts from human generated ones. 
Since it is time-consuming and costly to 
 ask a human to talk to a model 
and give judgements,
we  train a machine evaluator
in place of the  human evaluator to d the human-generated dialogues and machine dialogues, and use it to signify 
 the general quality of the generated responses. 

Adversarial evaluation involves both  training and testing. 
At training time, the evaluator is trained to
label dialogues as machine-generated (negative) and  human-generated (positive). 
At test time, the trained evaluator is evaluated on a held-out dataset.
If the human-generated dialogues and machine-generated ones are indistinguishable, the model  will achieve 50 percent accuracy at test time.  
\paragraph{Adversarial Error}
We follow the \newcite{bowman2015generating} and report the 
 the adversarial error, which is the
gap between the ideal accuracy 
of the evaluator
(i.e., 50$\%$, which means the machine generated utterance is indistinguishable from the human generated utterance)  and the actual accuracy attained.

Existing evaluation metrics ----- e.g., word-overlap metrics such as BLEU and METEOR, or the recently proposed dialogue evaluation metric ADEM \cite{hey}, which learns to predict human evaluation score to input responses ----- all focus on single turn dialogue quality evaluation. We argue that a dialogue generation model can be more properly evaluated on multi-turn dialogues. 
This is comparable to  the Turing test, in which the human evaluator is asked to chat with the machine for five minutes rather than just a single turn. 
We therefore propose evaluating the model
using multi-turn dialogues generated 
 by having  two bots  talk with each other. 

We  report adversarial error scores
 on dialogues with different number of simulated turns (length), specifically, {\it adver-1}, {\it adver-2} and {\it adver-3}, where {\it adver-N} denotes
the 
adversarial error 
 of an evaluator trained on dialogues 
 between the two bots
 simulated for $N$ turns. Theoretically, the larger $N$ is, the easier it is for the discriminator to recognize a machine generated dialogue and thus the higher the adversarial error would be. 

\paragraph{Testing the Evaluator's Ability}
One caveat  with the adversarial evaluation methods is that 
it is model-dependent. 
We approximate the human evaluator in the Turing test with an automatic evaluator and assume that the automatic evaluator is perfect.
Unfortunately, this is not always true.
An imperfect automatic evaluator results in the following issue:
 the low accuracy of the discriminator indicates high quality of the responses since we think the generated responses are indistinguishable from the human ones. However, there is another factor that can lead to the low discriminative accuracy----a poor discriminative model. 
 Consider a  discriminator that always gives random labels or always gives the same label.
 Such an evaluator 
   always yields 0 adversarial error (accuracy is always 50 percent).  
\newcite{bowman2015generating} propose  two different discriminator models 
separately using {\it unigram} features and {\it neural} features. It is hard to tell which feature set is more reliable. 
Standard strategy to test the model on a held-out development set is not suited to this case, since a model that overfits the develop set is necessarily superior. 
~~\\~~\\
To deal with this issue, we propose setting up a few manually-invented situations to test the ability of the automatic evaluator.
 This can be thought of as setting up  examinations to test the ability of the human evaluator in the Turing test. 
We  report not only the {\it adversarial error},  but also the scores that the evaluator
achieves
 in these manually set-up test cases, indicating how much we can trust the reported {\it adversarial error}. 
 We develop scenarios in which we know  in advance how a perfect evaluator should behave, and then compare the adversarial error from a discriminative model with the gold-standard error. Scenarios we design include:
 \begin{tightitemize}
 \item We use human-generated dialogues as both positive examples and negative examples. A perfect evaluator should give an adversarial error of $0$ (classification error $50\%$), which is the gold-standard result.
  \item We use machine-generated dialogues as both positive examples and negative examples. A perfect evaluator should give an adversarial error of $0$ (classification error $50\%$).
 \item We use original human-generated dialogues as positive examples and dialogues 
 with responses being
  random utterances 
  as negative examples. A perfect evaluator should give an adversarial error of $50$ (classification error $100\%$).
 \item We use original human-generated dialogues as positive examples and dialogues with 
 responses replaced by the utterances coming right after the true responses. 
 A perfect evaluation is supposed to give an adversarial error of $50$ (classification error $100\%$).
\end{tightitemize}
The {\it Evaluator Reliability Error} is the average deviation of an evaluator's adversarial error
 from the gold-standard error in the above tasks. 
The smaller value it takes, the more reliable the evaluator is. 

\section{Experimental Results} 
In this section, 
we detail experimental results on adversarial error, N-choose-1 metric and human evaluation.  
We also 
contrast 
the statistics of the responses generated from various models with the real conversational dataset 
 to shed light on the deficiencies of existing response generation models and suggest path for improvement. 
 \begin{table*}
\small
\centering
\begin{tabular}{cccc|ccc}\hline
& \multicolumn{3} {c|} {Unigram} &  \multicolumn{3} {c} {Neural} \\\hline
Model& adver-1 &adver-2  &adver-3  & adver-1 &adver-2   &adver-3   \\\hline
Discriminator Reliability Error& 0.124&0.084&0.057&0.098&0.082&0.054 \\\hline
 \sts (BS)&  0.387 & 0.422& 0.460&    0.444&0.470&0.490 \\
  \sts (Sampling)&0.356&0.407&0.450&0.425&0.440&0.482 \\
 \sts (MMI)&0.307  &0.359 &0.438 & 0.358 & 0.417&0.477 \\
Adversarial (Single-Turn)&0.275&0.340&0.428&0.310&0.375&0.465\\
Adversarial (Two-Turns)&0.270&0.316&0.404&0.291&0.349&0.435 \\
Adversarial (Three-Turns)&0.294&0.310&0.398&0.302&0.338&0.422\\\hline
\end{tabular}
\caption{Adversarial Error for different models.}
\label{adver}
\end{table*}

\subsection{Adversarial Evaluation}
As in \newcite{bowman2015generating}, we train two adversarial evaluation models using: (1)  unigram features and (2) a hierarchical encoder-model with a similar structure with the discriminator used in the reinforcement learning. 
We report adversarial error from the proposed model, along with baselines including standard $\sts$ models (beam-search and sampling), and the mutual information model \cite{li2015diversity}. Results are shown in Table \ref{adver}.  

First, according to the {\it Evaluator Reliability Error} shown in the first row of Table \ref{adver}, the 
results from the neural evaluator is generally more reliable than the unigram evaluator. Also, the 
evaluator  becomes more reliable as the number of simulated turns increases. 

The proposed adversarial training model yields better adversarial error scores than the  baselines. 
Interestingly, we find that {\it sampling} generally performs  better than beam search, indicating that
the
  distribution of the sampled responses is more similar to the real conversations than  the global optimal responses based on the model. 
This is similar to phenomenon reported in \shortcite{li2015diversity} that greedy decoding yields better results than beam-search. 
All  models perform poorly on {\it adver-3} evaluation metric, with the best adversarial error being 0.422, which means that the trained evaluator is  able to correctly distinguish between human-generated and machine generated dialogues with an accuracy more than 90 percent. 

We observe a performance boost from the {\it two-turn} adversarial model over the {\it single-turn} model. 
The explanation is that the dull generic responses (e.g., ``I don't know what you talking about") are commonly found in the training set. If we are doing single-turn simulation, it might confuse the discriminator in terms of whether to label the dull responses as positive or negative. 
 But it is very rare that the two consecutive turns in a normal conversation are both dull and generic. The  discriminator in the two-turn simulation can thus more confidently assign negative rewards to the commonplace simulated instances. As the reward is back-propagated to the generative model, the probability of generating dull responses will be pushed down for both turns.
We do not see a significant performance boost yielded by the {\it three-turn} simulation strategy 
over the 
 {\it two-turn}. The performance even deteriorates as the number of the simulated turns surpasses three. We suspect that this is because (1) the number of actions   grows linearly with the number the simulated turns. The system becomes harder and harder to train as the sequence of actions becomes longer and 
(2) The discriminator is too much more powerful than the generator as the number of the simulated turns becomes larger. The results for {\it four-turn} simulation is thus omitted for brevity. 

\subsection{N-choose-1 Metric}
We evaluate the model using N-choose 1 metric, as described in \newcite{shao15}. 
 In
the N-choose-1 evaluation, given dialogue history, we ask the model to rank N candidate responses, where one of the N candidate responses is the ground truth and the rest are random responses. 
We report 50, 10, 2-choose-1 accuracy. Results are shown in Table \ref{choose}. 
We see a clear performance boost from the adversarial model. 

\begin{table}
\small
\centering
\begin{tabular}{cccc}
Model&50&10&2\\\hline
\sts&0.087&0.24&0.62 \\
MMI&0.43&0.69&0.88\\
Adversarial&0.58&0.78&0.95\\\hline
\end{tabular}
\caption{N-choose-1 evaluation on different models.}
\label{choose}
\end{table}


\subsection{Human Evaluation}
For the human evaluation, we follow protocols defined in \newcite{li2016deep} where we employ
crowdsourced judges to evaluate a random sample of
200 items. We present both an input message and the
generated outputs to 3 judges and ask them to decide
which of the two outputs is better (denoted as single turn
general quality). Ties are permitted. Identical
strings are assigned the same score. 
For the second setting, judges are presented with simulated
conversations between the two agents (denoted
as multi-turn). Each conversation
consists of 3 turns.
Results are presented in Table \ref{human}.
We observe a significant quality improvement on both 
single-turn quality and multi-turn quality.
It is worth noting that the reinforcement learning system described in \newcite{li2016deep} which is optimized using human-defined rewards by having two agents talk with each other only yields better results on multi-turn dialogue quality, but not the single-turn. This confirms that the reward adopted in adversarial training, namely how indistinguishable is a machine-generated response from human-generated response, is a more general, natural and effective reward than manually defined rewards such as informativeness, ease of answering defined in  \newcite{li2016deep}.


\begin{table}
\small
\centering
\begin{tabular}{cccc}\\\hline
Setting &RL-win &RL-lose &Tie\\
single-turn& 0.62& 0.18 &0.20 \\
multi-turn& 0.72 &0.10& 0.18\\\hline
\end{tabular}
\caption{The gain
from the proposed adversarial model
 over the mutual information system
based on pairwise human judgments.}
\label{human}
\end{table}


\subsection{Statistics and Analysis}
In this subsection, we 
contrast the statistics of responses generated from different models with responses from human generated datasets.
Based on the statistics, we discuss the deficiencies of existing dialogue generation models and point out path for improvement. 


\begin{table}
\centering
\small
\begin{tabular}{cl}
Data Source& Ave Length \\\hline
Original& 11.7 \\
\sts (beam-search)&7.3   \\
\sts (MMI reranking)&8.9 \\
\sts (sampling)&9.2 \\
Adversarial (Single-Turn)& 9.5 \\
Adversarial (Two-Turns)& 10.0 \\\hline
\end{tabular}
\caption{Average response length for samples from the original  training set and responses generated from various models.}
\label{length}
\end{table}

\begin{table}
\centering
\small
\begin{tabular}{cl}
Data Source&Distinct-1  \\\hline
Original& 0.041 \\
\sts (beam-search)&0.0054   \\
\sts (MMI reranking)&0.013 \\
\sts (sampling)&0.031 \\
Adversarial (Single Turn)&0.026 \\
Adversarial (Two-Turns)&0.029 \\\hline
\end{tabular}
\caption{Diversity scores for samples from the original  training set and single-turn responses from various models.}
\label{diversity11}
 \end{table}

\begin{table}
\centering
\small
\begin{tabular}{cl}
Data Source&Ppl  \\\hline
Original& 42.4 \\
\sts (beam-search)&4.48   \\
\sts (MMI reranking)&11.4 \\
\sts (sampling)&34.6 \\
Adversarial (Single Turn)&33.5 \\
Adversarial (Two-Turn)&33.8 \\
\hline
\end{tabular}
\caption{Average response length from different sources.}
\label{ppl}
\end{table}

\begin{table*}[!ht]
\centering
\small
\begin{tabular}{ll}\hline
{\bf Input}: &You haven't been given an assignment in this case. \\
 vanilla \sts&  I don't know what you are talking about.\\
 mutual information& I've been looking all over for you. \\
 Sampling(1)& You 're gonna have to leave. \\
 Sampling(2)& You want your father back? \\
  Sampling(3)& Me? \\
   Sampling(4)&That 's right . \\
   Adversarial & You 've got one hell of a nerve . \\
 \hline
 {\bf Input}: & He is the one behind this scheme. \\
 vanilla \sts&   I don't know what you are talking about. \\
 mutual information& Yes, he is, isn't he?\\ 
  Sampling(1)& Still dwelling on that little problem , i think \\
  Sampling(2)& Not him ! \\
    Sampling(3)&  Well , it 's nice to meet you ! \\
    Sampling(4)&To drink through UNK UNK.  \\
Adversarial& and I was very angry at him for making me jumpy \\\hline
    {\bf Input}:   Have you heard of turing ? \\
     vanilla \sts&   No.\\
     mutual information&  Sure. \\
      Sampling(1)&The UNK 's theory of relativity is that i 'm a craftsman . \\
            Sampling(2)&No . \\
Sampling(3)&Oh my god ! \\
Sampling(4)&UNK ! \\
     Adversarial&  No. Have you ever heard of him ? \\\hline
\end{tabular}
\caption{
Single-turn dialogue simulation.}
\label{Single-turn}
\end{table*}

\begin{table*}
\centering
\small
\begin{tabular}{l|l}\hline
{\bf the Mutual Information Model}  & {\bf the Adversarial Model } \\\hline
{\bf Input}: {Do you love me ?} (1)             & {\bf Input}: Do you love me ? (1)   \\
\textsc{B}: {Yes, of course}. (2)    & B: More than anything in this world .\\
\textsc{A}: {I love you too.} (3)			    & A: Then we can stay together, you and me . (3) \\
\textsc{B}: {Goodbye, honey}. (4)			    & B: Yes , we can . (4) \\\hline
{\bf Input}: {Where are you going ?} (1)   & {\bf Input}: {Where are you going ?} (1)   \\
A: I am going to the restroom &B:   I 'm going to join the Army.\\
B: See you later. &A: You 're joking !\\
A: See you later. &B: No I'm not.\\\hline
\end{tabular}	
\caption{
Multi-turn dialogue simulation. The first turn (index 1) is input by the authors. Then the two agents take turns conversing, taking as input the other agent's prior generated turn. {\bf Left Column}: the mutual information reranking model. {\bf Right Column}: Dialogue simulated using the proposed adversarial  reinforcement learning model.}
\label{multi}
\end{table*}

We report various statistics of response including
 (1) average perplexity in which we take a pre-trained \sts model and compute  the average perplexity of the generated sequences given the input; 
 (2) response length and (3) the number of distinct unigrams in the generated responses 
 scaled by the total number of generated tokens.\footnote{We use the development set which contains roughly 10,000 examples. The examples in the dev-set are randomly sampled. } This scaling is to avoid favoring long sentences. 
Results are  shown in Tables \ref{length}, \ref{diversity11} and \ref{ppl}. 

We observe a surprisingly huge discrepancy between
the 
responses in the
true dataset and responses generated by the
 \sts model with beam-search, which intends to maximize the probability of the true dataset during training, and generates sequences with the largest probability at test time.  
 For example, 
 the decoded responses using beam-search yield an order of magnitude
 of smaller
  perplexity value (4.48) than the gold-standard references (42.4).\footnote{Such a big discrepancy is seldom observed  in
  other generation tasks such as 
  machine translation or image caption generation. For example, a trained attention model that shares similar structure on IWSLT 2015 English-German translation data yields a perplexity of 8.14 and 8.30 on the references and decoded outputs using the develop set.
The difference between 
tasks like machine translation or image caption generation 
 and response generation stems from the fact that 
the semantic needed to generated a target sequence is completely given by the input source. In contrast, in response generation, there are a great variety of answers to the dialogue inputs. 
And the beam search algorithm always generate the safest responses, which are mostly dull, generic and uninformative. }
The explanation is as follows:
generic responses form a small plurality with a long tail of diverse alternatives.
Responses are all alike whereas  response is diverse in its own way (quoted from {\it Anna Karenina}). This is high probability to generic response and thus results in 
beam-search decoding being dominated  by generic responses. 

 

Sampling at decoding time generates responses with distribution that more resemble the true training set. 
However, we find that sampled
responses are usually incoherent or sometime even ungrammatical. This is because the error accumulates as decoding goes on. A similar phenomenon has also been observed by \newcite{shao15}. 




For all of the three cases, in terms of the resemblance to the real distribution, the results from the adversarial model lie between sampling and beam-search model.  
Tables \ref{Single-turn} and \ref{multi} present
results from 
 single-turn and multi-turn simulations using the vanilla \sts model with beam search and sampling, mutual information model with beam-search and the proposed adversarial model. Inputs are borrowed from \newcite{li2015diversity,shao15} and not cherry-picked. It is interesting to see that some of the examples from 
sampling are of very high quality. However,  the response quality variance
for responses generated from sampling
 is pretty large. 
Generally, we observe that the proposed adversarial model tends to generate longer, more interesting and more coherent responses than the other baselines. 




\section{Conclusion and Future Work}
In this paper, drawing  intuitions from the Truing test, we propose to use adversarial training approach for response generation. We cast the model under the framework of reinforcement learning where the generator is trained based on the signal from the discriminator to generate response sequences indistinguishable from human-generated dialogues.
We observe a clear performance boost from the adversarial training strategy.

The adversarial training model should theoretically benefit a variety of generation tasks in NLP. Unfortunately, we apply the same training paradigm to machine translation but does not observe a performance boost. We conjecture that this is because the adversarial training strategy 
is more beneficial to
 tasks in which there is 
 a big discrepancy between the distributions of the generated sequences and the  reference target sequences. In other words,  more beneficial to the tasks in which entropy on the targets is  high. Exploring such a direction constitutes our future work. 
 ~~\\~~\\
 \noindent {\bf {\large Acknowledgements}}
The authors also want to thank Michel Galley, Bill Dolan, Chris Brockett, Jianfeng Gao 
and other members of the NLP group at Microsoft Research, as well as
 Sumit Chopra and Marc'Aurelio Ranzato from the Facebook AI Research for helpful discussions and comments. 
Jiwei Li is supported by a Facebook Fellowship,  which we gratefully acknowledge. 
This work is partially supported by the DARPA Communicating
with Computers (CwC) program under ARO prime
contract no. W911NF- 15-1-0462. Any opinions,
findings, and conclusions or recommendations expressed
in this material are those of the authors and
do not necessarily reflect the views of DARPA
or Facebook.


==> 04-simulation.tex <==
The central idea behind our approach is to simulate the process of two virtual agents taking turns talking with each other, through which we can explore the state-action space and learn a policy
$p_{RL}(p_{i+1}|p_{i}, q_i)$ that leads to the optimal expected reward.
We adopt an AlphaGo-style strategy \cite{silver2016mastering} by initializing the RL system using a general response generation policy which is learned from a fully supervised setting. 
\subsection{Supervised Learning}
 For the first stage of training, we build on prior work of predicting a generated target sequence given dialogue history using the supervised \sts model \cite{vinyals2015neural}.
 Results from supervised models will be later used for initialization. 
 
We trained a \sts model with attention \cite{bahdanau2014neural} on the OpenSubtitles dataset, which consists of roughly 80 million source-target pairs. 
We treated each turn in the dataset as a target and the concatenation of two previous sentences as source inputs. 
\subsection{Mutual Information}
Samples from \sts models are often times dull and generic, e.g., ``{\it i don't know}" \cite{li2015diversity}
We thus do not want to initialize the policy model using the pre-trained \sts models because this will lead to a lack of diversity in the RL models' experiences. 
 \newcite{li2015diversity} showed that modeling mutual information between sources and targets will significantly decrease the chance of generating dull responses and improve  general response quality.
We now show how we can obtain an encoder-decoder model which generates maximum mutual information responses. 


 
\begin{comment}  
For any pair of source $s=[p_i,q_i]$ and target $\hat{t}=p_{i+1}$, the mutual information between them is given by:
\begin{equation}
\begin{aligned}
m(p_{i+1}||q_{i},p_i)=\lambda\log p_{\sts}(p_{i+1}|p_i,q_i)\\
+(1-\lambda)\log p_{\sts}(q_i|p_{i+1})
\end{aligned}
\label{MMI}
\end{equation}

$\lambda$ denotes the trade-off between the probabilities of sources-given-targets and targets-given-sources and is set to 0.5. 
\end{comment}
As illustrated in \newcite{li2015diversity}, direct decoding from Eq~\ref{eq4} is infeasible since the second term 
 requires
 the target sentence to be  completely generated.
 Inspired by recent work on sequence level learning \cite{ranzato2015sequence}, we treat the problem of 
generating maximum mutual information response 
as a reinforcement learning problem in which a reward of mutual information value is observed when the model arrives at the end of  a sequence. 

Similar to \newcite{ranzato2015sequence}, we use policy gradient methods \cite{sutton1999policy,williams1992simple} for optimization. We initialize the policy model $p_{RL}$ using a pre-trained $p_{\sts}(a|p_i,q_i)$ model. 
Given an input source $[p_i,q_i]$, 
we generate a candidate list  $A=\{\hat{a}|\hat{a}\sim p_{RL}\}$. 
For each generated candidate $\hat{a}$, we will obtain the mutual information score $m(\hat{a}, [p_i,q_i])$ from the pre-trained $p_{\sts}(a|p_i,q_i)$ and $p^{\text{backward}}_{\sts}(q_i|a)$.
This mutual information score will be used as a reward and back-propagated to the encoder-decoder model, tailoring it to generate sequences with higher rewards. 
We refer the readers to \newcite{zaremba2015reinforcement}  and
\newcite{williams1992simple} for details.  The expected reward for a sequence is given by:
\begin{equation}
\begin{aligned}
&J(\theta)=\mathbb{E} [m(\hat{a},[p_i,q_i]) ]\\
\end{aligned}
\end{equation}
The gradient is
estimated using the likelihood ratio trick:
\begin{equation}
\begin{aligned}
\nabla J(\theta)=m(\hat{a},[p_i,q_i])\nabla\log p_{RL}(\hat{a}|[p_i,q_i])
\end{aligned}
\end{equation}
We update the parameters in the encoder-decoder model using stochastic gradient descent. 
A
curriculum learning strategy is adopted \cite{bengio2009curriculum} 
as in \newcite{ranzato2015sequence}  
such that, for
every sequence of length $T$ we use the MLE loss for the first $L$ tokens and the reinforcement algorithm for the remaining $T-L$ tokens. We gradually anneal 
the value of $L$ to zero.
A baseline strategy is employed to decrease the learning variance:
an additional neural model takes as inputs the generated target and the initial source and outputs a baseline value, similar to the strategy 
adopted by \newcite{zaremba2015reinforcement}. 
 The final gradient is thus:
\begin{equation}
\begin{aligned}
\nabla J(\theta)=\nabla\log p_{RL}(\hat{a}|[p_i,q_i]) [m(\hat{a},[p_i,q_i])-b]
\end{aligned}
\end{equation}


\subsection{Dialogue Simulation between Two Agents}
\label{sec:learning}
We simulate conversations between the two virtual agents and 
have them take turns talking with each other. The simulation proceeds as follows: at the initial step, a message from the training set is fed to the first agent. The agent encodes the input message to a vector representation and starts decoding to generate  a response output. 
Combining the immediate output from the first agent with the dialogue history, the second agent updates the state by encoding the dialogue history into a representation and uses the decoder RNN to generate responses, which are subsequently fed back to the first agent, and the process is repeated. 

\begin{figure*}[!ht]
    \centering
    %\includegraphics[width=6in]{2.png}
    \includegraphics[width=6in]{simulate-crop.pdf}
\caption{Dialogue simulation between the two agents. }
\end{figure*}



\paragraph{Optimization}
We initialize the policy model $p_{RL}$ with parameters from the mutual information model described in the previous subsection. 
We then use policy gradient methods to find parameters that lead to a larger expected reward.
%AR: Changed to address comment from reviewer #1
%For a sequence of actions $\{a_1, a_2, ..., a_T\}$, the reward function is given by:
The objective to maximize is the expected future reward:
\begin{equation}
%L=\mathbb{E} [ \sum_{i=1}^{i=T} R(a_i,[p_i,q_i] ) ]
J_{RL}(\theta)=\mathbb{E}_{p_{RL}(a_{1:T})} [ \sum_{i=1}^{i=T} R(a_i,[p_i,q_i] ) ]
\end{equation}
where $R(a_i,[p_i,q_i])$ denotes the reward resulting from action $a_i$. 
We
use the likelihood ratio trick 
\cite{williams1992simple,glynn1990likelihood,aleksand1968stochastic} for gradient updates:
\begin{equation}
%\nabla J(\theta)={ \sum_{i}\nabla\log p(a_i|p_i,q_i)} \sum_{i=1}^{i=T} R(a_i,[p_i,q_i] )
%AR: I think this is an approximation by sampling?
\nabla J_{RL}(\theta) \approx { \sum_{i}\nabla\log p(a_i|p_i,q_i)} \sum_{i=1}^{i=T} R(a_i,[p_i,q_i] )
\end{equation}

\begin{comment}
Baseline strategy is employed, which is standardly employed in training policy gradient model due to the huge variance values where 
\begin{equation}
\frac{\partial{L}}{\partial{\theta}}=\frac{\partial\sum_{i}\log p(a_i|p_i,q_i)}{\partial\theta} \sum_{i=1}^{i=T} (R(a_i,[p_i,q_i] )-b)
\end{equation}
\begin{equation}
b=\frac{{\partial\sum_{i}\log p(a_i|p_i,q_i)} \sum_{i=1}^{i=T} R(a_i,[p_i,q_i] )}{ \partial\sum_{i}\log p(a_i|p_i,q_i)}
\end{equation}
\end{comment}
We  refer readers to
\newcite{williams1992simple} and \newcite{glynn1990likelihood} for more details. 
\begin{comment}
For each simulated instance, we generate 5 candidate for each dialogue term. 
Since most of the generated translations in the N-best list are similar, differing only by punctuation or minor
morphological variations, candidates are generated by sampling from the distribution with additional Gaussian noise to foster more diverse candidates. 
\end{comment}

\begin{comment}
\begin{equation}
\begin{aligned}
\text{Loss}=&- \mathbb{E}_{a} [ \hat{R}(a,[p_i,q_i] ) ]\\
=&-\sum_{a} p_{RL}(a|p_i,q_i) [ \hat{R}(a,[p_i,q_i]) ]
\end{aligned}
\end{equation}
where $\hat{R}(a,[p_i,q_i])$ denotes future expected reward resulting from action $a$. $\hat{R}(a,[p_i,q_i])$ consists of two parts,
the immediate reward  $r(a,[p_i,q_i])$ observed from action $a$ computed using Eq~\ref{reward}  
and 
the value of future reward denoted as $r_{\text{future}}(a,[p_i,q_i])$ , 
which is equivalent to the expectation of the reward introduced by the sequence $a'$ generated from the other agent in response to  $a$.
 
 
\begin{equation}
r_{\text{future}}(a,[p_i,q_i])=\mathbb{E}_{a'} [ \hat{R}(a',[q_i,a])] 
\label{eq5}
\end{equation}
In Eq~\ref{eq5}, $[q_i,a]$ denotes the new state the system arrives after taking the action $a$, which is represented by the two consecutive dialogue turns $a$ and $q_i$.
We therefore have 
\begin{equation}
\begin{aligned}
\text{Loss}=&- \mathbb{E}_{a} [ \hat{R}(a,[p_i,q_i] ) ]\\
=& -\sum_{a} p_{RL}(a|p_i,q_i) r(a,[p_i,q_i])\\
-&\gamma\sum_{a} p_{RL}(a|p_i,q_i)\sum_{a'} \hat{R}(a',[q_i,a])
\end{aligned}
\label{eq6}
\end{equation}
where $\gamma$ denotes the discount factor and is set to 0.99. 
Two practical issues arise regarding Eq~\ref{eq6}. First, computing reward expectation requires summing over all possible actions which is infeasible given the infinite number of response candidates. 
We turn to a simplified strategy which approximates the entire action space by sampling a small list of candidates, denoted as C. $\mathbb{E}_{a} [ \hat{R}(a,[p_i,q_i] ) ] $ can then be rewritten as:
\begin{equation}
\begin{aligned}
& \mathbb{E}_{a} [ \hat{R}(a,[p_i,q_i] ) ]\\
&~~~~~~~~~~~~~ \approx \sum_{a\in C} \frac{p_{RL}(a|p_i,q_i)}{\sum_{a*\in C} p_{RL}(a|p_i,q_i)} [ \hat{R}(a,[p_i,q_i]) ]
\end{aligned}
\label{eq7}
\end{equation}
To avoid favoring shorter sequences, we replace $p_{RL}(a|p_i,q_i)$ with $p'_{RL}(a|p_i,q_i)$ which is the geometric mean of word-predicting probability:
\begin{equation}
p'_{RL}(a|p_i,q_i)=[p_{RL}(a|p_i,q_i)]^{1/N_a}
\end{equation}
where $N_a$ denotes the length of the generated sequence. 
Eq~\ref{eq7} is differentiable and gradients can be computed using standard back-propagation techniques. We refer the readers to the appendix for the full derivation of the objective function.

Since most of the generated translations in the N-best list are similar, differing only by punctuation or minor
morphological variations, candidates are generated by sampling from the distribution with additional Gaussian noise to foster more diverse candidates. 
\end{comment}
\subsection{Curriculum Learning}
A curriculum Learning strategy is again employed  in which we begin by simulating the dialogue for 2 turns, and gradually increase the number of simulated turns. 
We generate 5 turns at most, as  the number of candidates to examine grows exponentially in the size of candidate list.
Five candidate responses are generated at each step of the simulation.


==> 05-experiment.tex <==
In this section, we  describe experimental results along with qualitative analysis.  We evaluate dialogue generation systems using both human judgments and
two automatic metrics: conversation length (number of turns in the entire session) and diversity.
\subsection{Dataset}
The dialogue simulation requires  high-quality initial inputs fed to the agent. For example, an initial input of ``why ?" is undesirable since it is unclear how the dialogue could proceed. 
We take a subset of 10 million messages from the OpenSubtitles dataset and extract 0.8 million sequences with the lowest likelihood of generating the response
``{\it i don't know what you are taking about}" to ensure initial inputs are easy to respond to.


\subsection{Automatic Evaluation}
Evaluating dialogue systems is difficult. Metrics such as BLEU
\cite{papineni2002bleu} and perplexity have been widely used for
dialogue quality evaluation
\cite{li2015diversity,vinyals2015neural,sordoni2015neural}, but it
is widely debated how well these automatic metrics are correlated
with true response quality \cite{liu2016not,galley2015deltableu}.
Since the goal of the proposed system is not to predict the highest probability response, but rather the long-term success of the dialogue, 
we do not employ BLEU or perplexity for evaluation\footnote{We found the RL model performs worse on BLEU score. On a random sample of 2,500 conversational pairs, single reference BLEU scores for RL models, mutual information models and vanilla \sts models  are respectively 1.28, 1.44 and 1.17.  BLEU is highly correlated with perplexity in generation tasks. Since the RL model is trained based on future reward rather than MLE, it is not surprising that the RL based models achieve lower BLEU score.}. 

 
\paragraph{Length of the dialogue}
The first metric we propose is the length of the simulated dialogue. We say a dialogue ends when one of the agents starts generating dull responses such as ``{\it i don't know}" \footnote{We use a simple rule matching method, with a list of 8 phrases that count as dull responses.  Although this can lead to both false-positives and -negatives, it works pretty well in practice. }
or two consecutive utterances from the same user are highly overlapping\footnote{Two utterances are considered to be repetitive if they share more than 80 percent of their words.}. 


%We acknowledge the problems with the proposed evaluation metric. The success of the metric is predicated on the assumption that the simulated dialogue is already meaningful and coherent, which is  not always true. The two agents can always produce random sequences that are not semantically related to ``{\it i don't know}" and get high evaluation score.  Despite the shortcoming, the metric
%captures one specific aspect of 
% the long-term successfulness of dialogues and the capability of models that generate them. 

The test set consists of 1,000 input messages. 
To reduce the risk of circular dialogues, we limit the number of simulated turns to be less than 8.  
Results are shown in Table \ref{numturns}. As can be seen, using mutual information leads to more sustained conversations between the two agents.
The proposed  RL model is first trained based on the mutual information objective and thus benefits from it in addition to the RL model. 
We observe that the RL model with dialogue simulation achieves the best evaluation score. 


\begin{table}
\centering
\begin{tabular}{c|c}
Model& $\#$ of simulated turns \\\hline
\sts& 2.68 \\
mutual information& 3.40\\
RL&4.48 \\\hline
\end{tabular}
\caption{The average number of simulated turns from standard \sts models, mutual information model and the proposed RL model.}
\label{numturns}
\end{table}

\begin{table*}[!ht]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{lll}\hline
Input Message& Mutual Information Model& RL \\\hline
How old are you? & I'm 16. & I'm 16, why are you asking? \\
What's your full name? & I have no idea. & What's yours? \\
I don't want to go home tonight. & Really? & Why? \\
Do you have any feelings for me? & I don't know what you are talking about. &I don't want to hurt your feelings. \\
How much time do you have here? & Not long enough. Sorry, sir. & Ten seconds. \\
Shall we get started?& Of course! & Yes. We've got a lot of work to do here.\\
Do you play football? & No, i don't & Yes. I love football!\\ 
We'd have to talk to him.&I mean, he's a good guy&About what ? \\
How come you never say it? & Because I don't want to hurt you.& I don't think it's a good idea to say it. \\\hline
\end{tabular}
}
\caption{Sampled responses generated from the mutual information models and the proposed RL model.}
\label{sen}
\end{table*}


\begin{comment}
\begin{table}
\centering
\small
\begin{tabular}{l}\hline
\textsc{mutual information model}\\\hline
A: How old are you ? (initial input)\\
B: I'm 16.\\
A: 16 ? \\
B: I don't know what you are talking about. (end)\\\hline
\textsc{RL model}  \\\hline
A: How old are you ? (initial input)\\
B: I'm 16. Why are you asking ?\\
A: I thought you were 12. \\
B: What made you think so ? \\
A: I don't know what you are talking about. (end)\\\hline
\textsc{mutual information model}\\\hline
A: Where are you going ? (initial input)  \\
B: I 'm going to the restroom. \\
A: See you later. \\
B: See you later. \\
A: See you later. (end) \\\hline 
\textsc{RL model} \\\hline 
A: Where are you going ? (initial input)  \\
B: I 'm going to the police station .  \\
A: I 'll come with you . \\
B: no , no , no , no , you 're not going anywhere . \\
A: Why? \\
B: I need you to stay here. \\
A: I don't know what you are talking about.  (end) \\\hline
\end{tabular}
\caption{Simulated Conversation from Different Models. }
\label{simu}
\end{table}
\end{comment}

\paragraph{Diversity} 
We report degree of diversity by calculating
the number of distinct unigrams and bigrams
in generated responses. The value is scaled by the total
number of generated tokens to avoid favoring long
sentences as described in \newcite{li2015diversity}.
The resulting metric is thus a type-token ratio for unigrams and bigrams.

For both the standard \sts model and the proposed RL model, we use beam search with a beam size 10 to generate a response to a given input message. For the mutual information model, we first generate $n$-best lists using $p_{\sts}(t|s)$ and then linearly re-rank them using $p_{\sts}(s|t)$.
Results are presented in Table \ref{diversity}. We find that the proposed RL model generates more diverse outputs when compared against both the vanilla \sts model and the mutual information model. 

\begin{table}[ht]
\centering
\begin{tabular}{c|l|l}
Model& Unigram&Bigram \\\hline
\sts& 0.0062&0.015 \\
mutual information& 0.011&0.031\\
RL&0.017&0.041 \\\hline
\end{tabular}
\caption{Diversity scores (type-token ratios) for the standard \sts model, mutual information model and the proposed RL model.}
\label{diversity}
\end{table}



\paragraph{Human Evaluation}
We explore three settings for human evaluation:
the first setting is similar to what was described in \newcite{li2015diversity},
where we employ crowdsourced judges to evaluate a random sample of 500 items. 
We present both an input message and the generated outputs to 3 judges and ask them to 
 decide which of the two outputs is better (denoted as {\it single-turn general quality}). 
Ties are permitted. 
Identical strings are assigned the same score. 
We measure the improvement achieved by the RL model over the mutual information model by the mean difference in scores between the models. 

For the second setting, judges are again presented with input messages and system outputs, but are asked to decide which of the two outputs is easier to respond to (denoted as {\it single-turn ease to answer}).
Again we evaluate a random sample of 500 items, each being assigned to 3 judges. 


For the third setting, judges are presented with simulated conversations between the two agents (denoted as {\it multi-turn general quality}). Each conversation consists of 5 turns. 
We evaluate 200 simulated conversations, each being assigned to 3 judges, who are asked to decide which of the simulated conversations is of higher quality.

\begin{table}[!ht]
\centering
\small
\begin{tabular}{cccc} \\\hline
Setting&RL-win&RL-lose&Tie  \\\hline
single-turn general quality&0.40&0.36&0.24 \\
single-turn ease to answer& 0.52&0.23&0.25\\
multi-turn general quality&0.72&0.12&0.16\\\hline
\end{tabular}
\caption{RL gains over the mutual information system based on pairwise human judgments.}
\label{human-eval}
\end{table}

Results for human evaluation are shown in Table \ref{human-eval}. 
The proposed RL system does not introduce a significant boost in single-turn response quality (winning 40 percent of time and losing 36 percent of time).
This is in line with our expectations, 
as the RL model is not optimized to predict the next utterance, but rather to increase long-term reward.
The RL system produces responses that are significantly easier to answer than 
does the mutual information system, as demonstrated by the {\it single-turn ease to answer} setting (winning 52 percent of time and losing 23 percent of time),
and also significantly higher quality multi-turn dialogues, as demonstrated by the {\it multi-turn general quality} setting (winning 72 percent of time).


\paragraph{Qualitative Analysis and Discussion}
We show a random sample of generated responses in Table \ref{sen} and simulated conversations in Table \ref{con-simulation} at the beginning of the paper.
From Table \ref{sen}, we can see that the RL based agent indeed generates more interactive responses than the other baselines. We also find that the RL model has a tendency to 
end a sentence with another question and hand the conversation over to the user. 
From Table \ref{con-simulation}, we observe that the RL model manages to produce more interactive and sustained conversations than the mutual information model. 

During error analysis, we found that although we penalize repetitive utterances in consecutive turns, the dialogue sometimes enters a cycle with length greater than one, as shown in Table \ref{he}. This can be ascribed to the 
limited amount of conversational history we consider. 
Another issue observed is that the model sometimes starts a less relevant topic during the conversation. There is a tradeoff between relevance and less repetitiveness, as manifested in the reward function we define in Eq~4. 

\begin{table}[!ht]
\centering
\small
\begin{tabular}{l}\hline
A: What's your name ?\\
B: Daniel.  \\
A: How old are you ?\\
B. Twelve. What's your name ? \\
A. Daniel.  \\
B: How old are you ? \\
A: Twelve. What's your name ? \\
B: Daniel.\\
A: How old are you ? \\
B ... \\\hline
\end{tabular}
\caption{An simulated dialogue with a cycle longer than one.}
\label{he}
\end{table}

The fundamental problem, of course, is that the manually defined reward function 
can't possibly cover the crucial aspects that define an ideal conversation. 
While the heuristic rewards that we defined are amenable to automatic calculation,
and do capture some aspects of what makes a good conversation, ideally 
the system would instead receive real rewards from humans.
Another problem with the current model is that we can only afford to explore a very small number of candidates and simulated turns since the number of cases to consider grow exponentially. 
%How to handle these problems naturally constitute our future work. 

